Towards Valid and Reliable Privacy Concern Scales: The Example of IUIPC-8

Valid and reliable measurement instruments are crucial for human factors in privacy research. We expect them to measure what they purport to measure, yielding validity, and to measure this consistently, offering us reliability. While there is a range of privacy concern instruments available in the field and their investigation continues unabated, we shall focus on a brief form of the scale Internet Users? Information Privacy Concerns (IUIPC-8) as an example. We not only present IUIPC-8 itself, but also consider methods for the evaluation of valid and reliable measurement instruments. In this, confirmatory factor analysis (CFA) serves us as a valuable tool. Our inquiry takes into account the ordinal and non-normal data yielded by the IUIPC questionnaire, compares multiple models to confirm the three-dimensionality of the scale, examines global and local fit and, finally, estimates construct validity and internal consistency reliability metrics. We offer a comparison between IUIPC-10 and IUIPC-8 drawing on two independent samples. In conclusion, we highlight properties of the scale and considerations for its use in practice.

==> IUIPC-8_FA-concordance.tex <==
\Sconcordance{concordance:IUIPC-8_FA.tex:IUIPC-8_FA.Rnw:%
1 4 1 50 0 1 5 151 1 1334 0}


==> IUIPC_original_fit.tex <==
\begin{table}[tb]
\centering
\footnotesize
\caption{Fit of IUIPC-10's second-order model~\cite[p. 346]{malhotra2004internet}}
\label{tab:iuipc_original_fit}
\begin{tabular}{r@{ }r@{ }rrrr@{ }r}
  \toprule
$\chi^{2}$ & $\vari{df}$ & \textit{p} & \textsf{CFI} & \textsf{GFI} & \textsf{RMSEA} & $p_{\epsilon_0 \leq .05}$\\ 
  \midrule
73.19 & 32 & $< .001$ & $.98$ & $.97$ & .054 [.037, .070]  &  $.338$ \\
   \bottomrule
\end{tabular}
\\\emph{Note:} $N_{\mathsf{IUIPC}} = 449$. \textsf{RMSEA} with inferred 90\% CI. 
%\textsf{SRMR} was not reported in IUIPC~\cite{malhotra2004internet} and could not be computed.
\end{table}

==> Modeling_Approach.tex <==
\begin{table*}
\centering
\caption{Modeling approaches}
\begin{tabular}{rccc}
\toprule
    &   \multicolumn{3}{c}{Estimator}\\
    \cmidrule(lr){2-4}
                    & \multicolumn{2}{c}{Maximum Likelihood} & Weighted Least Squares\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4}
                     &  ML & MLM & WLSVM \\
\midrule
Scale            & Continuous & Continuous & Ordinal \\
Normality      & Normal  & Not extremely non-normal & Non-normal \\
Completeness & Not required & Complete only & Complete only \\
$\chi^2$ Test & Standard & Satorra-Bentler scaled & Satterthwaite mean/variance adjusted \\
$\vari{SE}$    & Standard & Robust & Robust \\
Interpretation & Linear & Linear & Probit \\
\bottomrule
\end{tabular}
\end{table*}

==> abstract.tex <==
Valid and reliable measurement instruments are crucial for human factors in privacy research. We expect them to measure what they purport to measure, yielding validity, and to measure this consistently, offering us reliability. While there is a range of privacy concern instruments available in the field and their investigation continues unabated, we shall focus on a brief form of the scale Internet Users? Information Privacy Concerns (IUIPC-8) as an example. We not only present IUIPC-8 itself, but also consider methods for the evaluation of valid and reliable measurement instruments. In this, confirmatory factor analysis (CFA) serves us as a valuable tool. Our inquiry takes into account the ordinal and non-normal data yielded by the IUIPC questionnaire, compares multiple models to confirm the three-dimensionality of the scale, examines global and local fit and, finally, estimates construct validity and internal consistency reliability metrics. We offer a comparison between IUIPC-10 and IUIPC-8 drawing on two independent samples. In conclusion, we highlight properties of the scale and considerations for its use in practice.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We independently evaluated the \refterm{validity}{validity} and \refterm{reliability}{reliability} of IUIPC-10 in covariance-based confirmatory factor analyses.
Acknowledging the sound content validity foundations presented by Malhotra et al.~\cite{malhotra2004internet} and the instrumental role the scale played in advancing the field, we observed that 
\begin{inparaenum}[(i)]
  \item we could confirm the three-dimensionality of IUIPC-10 with the factors \fName{Control}, \fName{Awareness}, and \fName{Collection},
  \item we found disconfirming evidence for the \refterm{factorial_validity}{factorial validity} and \refterm{convergent_validity}{convergent validity}, largely rooted in evidence against the \refterm{unidimensionality}{unidimensionality} of \fName{Control} and \fName{Awareness}. These results were consistent in main analysis and validation, irrespective of the estimator used,
  \item we proposed a respecified IUIPC-8 that outperformed the original IUIPC-10 on \refterm{construct_validity}{construct validity} and \refterm{reliability}{reliability} consistently. 
  \item we offered empirically grounded recommendations how to use IUIPC and similar privacy concern scales.
\end{inparaenum}

Future work specifically for IUIPC would ideally offer further carefully evaluated revisions to the scale, eliminating identified problems in question wording, e.g., eliminating loaded words, aiming for four items per factor, and establishing unassailable \refterm{construct_validity}{construct validity} and an internal consistency $\omega > .80$ for all sub-scales.

We started this paper referring to instruments as measuring stick for privacy concern.
If such a measurement stick is warped, the community's investigation of human factors of PETs and of the privacy paradox may be severely undermined and misled.
We believe that we would benefit from concerted efforts to diligently evaluate standard instruments in the field along similar lines we have pursued in this study.
While reaching consensus on sound measurement instruments on the construct \fName{Information Privacy Concern} and its siblings is essential, we would also benefit from following unified recommendations their use. 

==> limitations.tex <==
\subsection{Limitations}
\label{sec:limitations}

In terms of generalizability, this study encountered the usual limitations of self-report instruments, where we sought to ward against straightlining with instructional manipulation checks/attention checks. 
While the sampling aimed at representing a UK population, the sampling process was non-randomized and affected by a self-selection bias due to Prolific's matchmaking.

Factor analyses like ours are affected by sampling and measurement errors. To ensure our findings yielded cross-sample validity, we considered three independent samples. To ensure our findings were valid irrespective of design decisions, we created a direct replication of the IUIPC-10 as well as analyses following methodological recommendations~\cite[p. 122]{kline2012assumptions}. The results were invariant to outlier inclusion and estimation method.

==> refinedPathPlotV.tex <==

\newcommand{\pathPlotCFAVreduxwlsref}{
\begin{figure*}[tbp]
\centering
\includegraphics[keepaspectratio,width=0.8\maxwidth]{figure/cfaSEMPlotV-static} 
\caption{CFA paths plot with standardized estimates of IUIPC-8 on Sample \textsf{V}. \emph{Note:} The dashed lines signify that the raw factor loading was fixed to 1 (cf. Table~\ref{tab:loadingsVreduxwls}).}
\label{fig:pathPlotCFAVreduxwlsref}
\Description[The path plot of the IUIPC-8 model on the validation sample V showing the three first-level factors ctrl, aware, and collect and the second-level factor iuipc.]{This path plot shows the final IUIPC-8 model on validation sample V. On the bottom, we have eight indicator variables, for which vertical lines depict the thresholds of the WLSMV model. In the middle, we have the three first-level factors ctrl, aware, and collect. On the top, we show the second-level factor iuipc.}
\end{figure*}
}
